Decentralized Personalized Online Federated Learning

Vanilla federated learning does not support learning in an online environment, learning a personalized model on each client, and learning in a decentralized setting. There are existing methods extending federated learning in each of the three aspects. However, some important applications on enterprise edge servers (e.g. online item recommendation at global scale) involve the three aspects at the same time. Therefore, we propose a new learning setting \textit{Decentralized Personalized Online Federated Learning} that considers all the three aspects at the same time. In this new setting for learning, the first technical challenge is how to aggregate the shared model parameters from neighboring clients to obtain a personalized local model with good performance on each client. We propose to directly learn an aggregation by optimizing the performance of the local model with respect to the aggregation weights. This not only improves personalization of each local model but also helps the local model adapting to potential data shift by intelligently incorporating the right amount of information from its neighbors. The second challenge is how to select the neighbors for each client. We propose a peer selection method based on the learned aggregation weights enabling each client to select the most helpful neighbors and reduce communication cost at the same time. We verify the effectiveness and robustness of our proposed method on three real-world item recommendation datasets and one air quality prediction dataset.

==> old.tex <==


\section{Method}
\subsection{What to share?}
If we consider applications in Adobe, we will share learned parameters and not gradients, but we still have the question of share parameters from which epoch. Is converged parameters the best?

\subsection{Who to share?}
The who question makes sense mostly in p2p setting.
If we have a central or regional server, do we fetch aggregated model from which server or fetch the local model of other devices through the server?

Learning to discover a graph for personalization. Each devices finds out the devices have similar data distribution and share/fetch information to/from these devices. 

A model $h$ is learned to measure the similarity between a device $i$ and it's neighboring nodes. 
Each device keeps a list of its $K$ most similar neighbors (ranked use $h$).

randomized search to discover similar neighbors: for device $i$, we want to update its $K$ neighbors. Randomly pick one from the $K$ neighbors, get one neighbor of the picked one. Add it to the neighbors of device $i$ if similarity is higher than the least similar neighbors.


\subsection{When to share?}
We want to fetch information to improve the local model when (1) the local device has few data (2) there is a data shift.
Otherwise the local device has seen enough local data, so a good local model can be learned, and we don't need to fetch information so communication is reduced.



\subsection{How to combine?}
We consider the $i$th local device with local model $M_i$.
Each neighbor $j$ is associated with a feature vector $M_j^f$. The feature vector encodes information about the neighbor, including model performance on its local device, similarity of model parameters $sim(M_i, M_j)$, the number of epochs, the amount of data trained on.

We learn a model $g$ that takes in a feature vector $M_j^f$ and outputs a weight $w_j$, i.e. $w_j=g(M_j^f)$.  
The local model $M_i$ is then updated as:
\begin{equation}
    M_i' = \frac{1}{1+\sum_j w_j}(M_i+\sum_j w_j M_j)
\end{equation}
